Quantizable Transformers: Removing Outliers by Helping Attention Heads Do Nothing

Transformer models have been widely adopted in various domains over the last years, and especially large language models have advanced the field of AI significantly. Due to their size, the capability of these networks has increased tremendously, but this has come at the cost of a significant increase in necessary compute. Quantization is one of the most effective ways to reduce the computational time and memory consumption of neural networks. Many studies have shown, however, that modern transformer models tend to learn strong outliers in their activations, making them difficult to quantize. To retain acceptable performance, the existence of these outliers requires activations to be in higher bitwidth or the use of different numeric formats, extra fine-tuning, or other workarounds. We show that strong outliers are related to very specific behavior of attention heads that try to learn a "no-op" or just a partial update of the residual. To achieve the exact zeros needed in the attention matrix for a no-update, the input to the softmax is pushed to be larger and larger during training, causing outliers in other parts of the network. Based on these observations, we propose two simple (independent) modifications to the attention mechanism - clipped softmax and gated attention. We empirically show that models pre-trained using our methods learn significantly smaller outliers while maintaining and sometimes even improving the floating-point task performance. This enables us to quantize transformers to full INT8 quantization of the activations without any additional effort. We demonstrate the effectiveness of our methods on both language models (BERT, OPT) and vision transformers.

==> figures/_archive/post_LN_vs_pre_LN.tex <==
See Figure~\ref{fig:02_transformer_layer_LN}.
% 
% ## Figure transformer layer so we can show where the outliers are + discuss LayerNorm placement
% 
\begin{figure*}[htb]
\subfloat[Post-LN]{
    \label{fig:02_transformer_layer_post_LN}
    \includegraphics[width=.25\textwidth]{img/02_post_LN.png}
}
\qquad
\qquad
\subfloat[Pre-LN]{
    \label{fig:02_transformer_layer_pre_LN}
    \includegraphics[width=.25\textwidth]{img/02_pre_LN.png}
}
% 
\centering
\vspace{-.1cm}
\caption{%
A schematic illustration of the transformer layer with different LayerNorm placements.
% \protect\subref{fig:02_transformer_layer_post_LN}
% \protect\subref{fig:02_transformer_layer_pre_LN} Pre-LN placement.
\todo{MN: The figures are nice, but IMO not as crucial to justify that much space.}
\label{fig:02_transformer_layer_LN}
\end{figure*}


==> rebuttal/figure_bert_attention_patterns.tex <==
\begin{figure*}[htb]

% # -- Vanilla --
\subfloat[Vanilla softmax (Attention layer \#11, head \#3, data sequence \#5)]{
    \label{fig:bert_attention_vanilla}
    \includegraphics[width=.13\textwidth]{img/03_bert_attention/P2.png}
    \;
    \includegraphics[width=.38\textwidth]{img/03_bert_attention/V2.png}
    \;
    \includegraphics[width=.38\textwidth]{img/03_bert_attention/PV2.png}
}
\\
\vspace{-.1cm}
% # -- Clipped softmax --
\subfloat[Clipped softmax (Attention layer \#11, head \#1, data sequence \#7)]{
    \label{fig:bert_attention_clipped_softmax}
    \includegraphics[width=.155\textwidth]{img/rebuttal_bert_attention_clipped_softmax/P.png}
    \;
    \includegraphics[width=.37\textwidth]{img/rebuttal_bert_attention_clipped_softmax/V.png}
    \;
    \includegraphics[width=.37\textwidth]{img/rebuttal_bert_attention_clipped_softmax/PV.png}
}
\\
\vspace{-.1cm}
% # -- Gated attention --
\subfloat[Gated attention (Attention layer \#11, head \#1, data sequence \#1)]{
    \label{fig:bert_attention_gating}
    \includegraphics[width=.055\textwidth]{img/rebuttal_bert_attention_gating/PI.png}
    \;
    \includegraphics[width=.135\textwidth]{img/rebuttal_bert_attention_gating/P.png}
    \;
    \includegraphics[width=.38\textwidth]{img/rebuttal_bert_attention_gating/V.png}
    \;
    \includegraphics[width=.38\textwidth]{img/rebuttal_bert_attention_gating/PI_PV.png}
}
%
\centering
% \vspace{-.1cm}
\caption{%
%
Visualization of the self-attention patterns for BERT-base trained using vanilla and our proposed techniques, computed on data sequences from MNLI-m validation set.
% 
\protect\subref{fig:bert_attention_vanilla},~\protect\subref{fig:bert_attention_clipped_softmax}: attention probabilities, values, and their product.
% 
\protect\subref{fig:bert_attention_gating}: gating probabilities $\bs{\pi} = \sigmoid\p{\G\p{\x}}$, attention probabilities (output of softmax), values, and their combined product.
}
\end{figure*}
% 


==> rebuttal/table_bert_low_bit_results.tex <==
\begin{table*}[htb]
    \centering
    \begin{tabular}{ ccccc }
        \toprule
        Bitwidths & Weight range estimation & Vanilla & Clipped softmax & Gated attention \\
        \midrule 
        FP16 & $-$ & \ms{4.49}{0.01} & \ms{4.39}{0.00} & \ms{4.45}{0.03} \\
        \midrule 
        W8A8 & min-max & \ms{1294}{1046} & \ms{4.52}{0.01} & \ms{4.65}{0.04} \\
        W6A8 & min-max & \ms{598}{254} & \ms{4.64}{0.01} & \ms{4.79}{0.03} \\
        W6A8 & MSE & \ms{6.49}{0.38} & \ms{4.56}{0.01} & \ms{4.71}{0.03} \\
        W4A8 & MSE & \ms{6.52}{0.02} & \ms{4.90}{0.02} & \ms{5.02}{0.03} \\
        W6A6 & MSE & \ms{42.8}{11.7} & \ms{6.64}{0.14} & \ms{5.90}{0.11} \\
        \bottomrule
    \end{tabular}
    \caption{
    % 
    A summary of results for our proposed methods applied to BERT-base and quantized to different bitwidthds for weights and activations (using the same PTQ setup as in all previous experiments). We report the masked language modeling perplexity on the English
Wikipedia validation set.
}
\end{table*}
% 
% 

==> rebuttal/table_opt_fine_tuning.tex <==
\begin{table*}[htb]
    \centering
    \begin{tabular}{ lccc }
        \toprule
        Method & FP16 ppl.$\da$ & Max inf norm & Avg. Kurtosis \\
        \midrule       
        Vanilla fine-tuning & 29.46 & 79.3 & 2086 \\
        Fine-tuning w/ Gated attention & 29.18 & 50.9 & 665 \\
        \bottomrule
    \end{tabular}
    % \vspace{-.cm}
    \caption{%
    % 
    OPT-1.3B fine-tuning results with vanilla softmax and Gated attention.
    % 
    We report the causal language modeling perplexity (ppl. for short) on the English Wikipedia validation set.
    %  
    We also report the maximum $\|\x\|_{\infty}$ averaged across the validation set, and kurtosis of $\x$ averaged across all layers, where $\x$ is the output of an attention layer.
}
\end{table*}


==> sections/_archive/_3_analysis_DRAFT.tex <==
\section{Outlier analysis and hypothesis}
\label{sec:analysis}

% ============================================================================================
% ---------------------------------------------------------------------------------------------


% Even more compact:
% \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
%   \item foo
%   \item bar
%   \item baz
% \end{itemize}


% \2 $\softmax\p{\x}_i > 1 - \varepsilon,\,\varepsilon>0$ (so that the rest of components sum up to at most $\varepsilon$), then the dynamic range $\x_{\text{max}} - \x_{\text{min}} = \x_i - \x_{\text{min}} \geq \x_i - \x_j > \ln\p{\frac{1 - \varepsilon}{\varepsilon}}$
%     % 
%     \todo{consider $\softmax\p{\x}_i < \varepsilon/d$}
    

% ---------------------------------------------------------------------------------------------


% ============================================================================================


% % #
% % ##
% % ### OPT
% % 
% \paragraph{Outlier analysis in OPT}
% % 
% We study the outliers properties and the relation to the attention patterns in the next layers for OPT.
% \todo{MN: Let's consider moving it to the appendix if we have not enough space or time to get it done.}


% Plan:
% \begin{outline}[itemize]
%  % 
%  \1 We train it ourselves (6 layer model) \todo{check for 12 layer model} (see details in Section~\ref{sec:experiments}). See Figure~\ref{fig:03_vit_attention}
%  % 
%  \1 significant portion of attention mass is allocated to the first token. THis is in line with the literature~\cite{vig-belinkov-2019-analyzing}.
%  % 
%  \1 values are not zero.
%  % 
%  \1 (why not zero might be related to the model capacity)
% \end{outline}
% % 
% % 
% \begin{figure*}[htb]
% \subfloat[]{
%     % \label{fig:03_opt_attention_outliers}
%     \includegraphics[width=.58\textwidth]{img/03_opt_attention/FFN.png}
% }
% \quad
% \subfloat[]{
%     % \label{fig:03_vit_attention_weights}
%     \includegraphics[width=.19\textwidth]{img/03_opt_attention/P.png}
% }
% \quad
% \subfloat[]{
%     % \label{fig:03_vit_attention_matrix}
%     \includegraphics[width=.14\textwidth]{img/03_opt_attention/V.png}
% }
% % 
% \centering
% \vspace{-.1cm}
% \caption{%
% % Visualization of the attention pattern and relation to outliers in 1st attention head of 12th layer in ViT-S/16, computed on an image from ImageNet-1K~\cite{imagenet} validation set.
% % % 
% % \protect\subref{fig:03_vit_attention_outliers} Visualization of outliers in the previous, 11th layer. Outliers are defined as channels that exceed 12 standard deviations from the mean of output of the layer.
% % % 
% % \protect\subref{fig:03_vit_attention_weights} A visualization of cumulative attention weight spent on every token (attention matrix summed over rows) in the next, 12th layer.
% % % 
% % \protect\subref{fig:03_vit_attention_matrix} A matrix of attention weights.
% % % 
% % \protect\subref{fig:03_vit_attention_values} Corresponding values for the same head.
% % 
% }
% \label{fig:03_opt_attention}
% \end{figure*}

% ============================================================================================



==> sections/_archive/_6_related_work.tex <==
\section{Related work}
\label{sec:related_work}

% ---------------------------------------------
% ===============================================================

// all the related work that is not related to outliers
%
\begin{itemize}
    %
    \item efficient transformer architectures, linear attention ....
    %
    \item pruning
    %
    \item ...
    %
\end{itemize}
%


==> sections/_archive/_8_broader_impact.tex <==


% ---------------------------------------------
% ===============================================================


==> tables/_archive/_05_ablation_vit_gated_attention.tex <==
\begin{table*}[htb]
    \centering
    \begin{tabular}{ cccccc }
        \toprule
         $G(\mathbf{x})$ & Bias init & Activation & FP32 acc. & Max inf norm & W8A8 acc. \\
         \midrule  
         $\nheads{}\times\linear(\dhead \ra 1)$ & random & sigmoid & \bf{78.20}\fstd{\bf{0.14}} & \bf{121}\fstd{\bf{31}}	& \bf{76.64}\fstd{\bf{0.37}} \\
         $\nheads{}\times\linear(\dhead \ra 1)$ & $\sigma^{-1}(0.75)$ & sigmoid & 77.91\fstd{0.14}	& 163\fstd{1}	& 74.99\fstd{0.56} \\
         $\nheads{}\times\linear(\dhead \ra 1)$ & $\sigma^{-1}(0.9)$ & sigmoid & 78.68\fstd{0.30}	& 283\fstd{10}	& 75.22\fstd{0.88} \\
         \midrule
         $\nheads{}\times\linear(\dhead \ra 1)$ & random & rect.~sigmoid ($t=0.003$) & 78.34\fstd{0.13}	& 130\fstd{42}	& 76.52\fstd{0.65} \\
         $\nheads{}\times\linear(\dhead \ra 1)$ & random & rect.~sigmoid ($t=0.01$) &78.27\fstd{0.15}	& 136\fstd{24}	& 76.00\fstd{0.57} \\
         $\nheads{}\times\linear(\dhead \ra 1)$ & random & rect.~sigmoid ($t=0.03$) &78.36\fstd{0.05}	& 161\fstd{54}	& 76.07\fstd{0.52} \\
         $\nheads{}\times\linear(\dhead \ra 1)$ & random & rect.~sigmoid ($t=0.1$) &78.02\fstd{0.36}	& 231\fstd{83}	& 74.42\fstd{0.53} \\
         \midrule
         $\nheads{}\times\mlp(\dhead \ra 4 \ra 1)$  & random & sigmoid & 78.36\fstd{0.02}	& 143\fstd{29}	& 76.24\fstd{0.61} \\
         $\nheads{}\times\mlp(\dhead \ra 64 \ra 1)$ & random & sigmoid & 78.37\fstd{0.43}	& 196\fstd{155}	& 75.80\fstd{0.41} \\
         $\linear(\dmodel \rightarrow \nheads)$     & random & sigmoid & 78.79\fstd{0.45}	& 338\fstd{65}	& 75.67\fstd{0.43} \\
         \midrule  
         \bottomrule
    \end{tabular}
    \vspace{-.1cm}
    \caption{A comparison of different architectural choices for gated attention applied to ViT-S/16.
    % 
    We report the top-1 accuracy on ImageNet-1K validation set for floating-point baseline and W8A8 quantized model.
    % 
    Max inf norm is the maximum infinity norm of the hidden activation, averaged over validation set.
    % 
    In all cases, we report an average $\pm{}$ standard deviation over 2 run with different random seeds
    % 
    $\sigma^{-1}(p)=\ln\p{\frac{p}{1 - p}}$ is the inverse sigmoid,
}
    \label{tbl:05_ablation_vit_gated_attention}
\end{table*}

